DiffSHEG: A Diffusion-Based Approach for Real-Time Speech-driven Holistic 3D Expression and Gesture Generation

We propose DiffSHEG, a Diffusion-based approach for Speech-driven Holistic 3D Expression and Gesture generation with arbitrary length. While previous works focused on co-speech gesture or expression generation individually, the joint generation of synchronized expressions and gestures remains barely explored. To address this, our diffusion-based co-speech motion generation transformer enables uni-directional information flow from expression to gesture, facilitating improved matching of joint expression-gesture distributions. Furthermore, we introduce an outpainting-based sampling strategy for arbitrary long sequence generation in diffusion models, offering flexibility and computational efficiency. Our method provides a practical solution that produces high-quality synchronized expression and gesture generation driven by speech. Evaluated on two public datasets, our approach achieves state-of-the-art performance both quantitatively and qualitatively. Additionally, a user study confirms the superiority of DiffSHEG over prior approaches. By enabling the real-time generation of expressive and synchronized motions, DiffSHEG showcases its potential for various applications in the development of digital humans and embodied agents.

==> cvpr_sec/4_figures.tex <==

%------------------------ figure only pages --------------
\clearpage

% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=0.99\linewidth]{fig/gesture_plus_head_diversity.pdf}
% \vspace{-0.5cm}
% \end{center}
%    \caption{\textbf{Motion Diversity Comparison of Models Trained on the SHOW~\cite{talkshow} Dataset.} Our method generates more expressive and diverse motions than TalkShow~\cite{talkshow} and LS3DCG~\cite{habibie2021learning} in terms of both gesture and head pose diversity. }
% \label{fig:motion_dieversity}
% \end{figure*}

% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=0.95\linewidth]{fig/head_and_expression.pdf}
% \vspace{-0.5cm}
% \end{center}
%    \caption{\textbf{Expression and Head Pose Comparison of Models Trained on the SHOW~\cite{talkshow} Dataset.}
%    (a) When provided with speech audio as input, TalkShow~\cite{talkshow} and LS3DCG~\cite{habibie2021learning} may generate unnatural and persistent head-down poses showing limited variation. In contrast, our method produces a wide range of expressive head poses. (b) Prior to the audio input's emphasis on the word ``five'', our approach instinctively raises the head to prepare for highlighting, subsequently producing precise lip movements accompanied by raised eyebrows to emphasize the word ``five''.
%    }
% \label{fig:head_and_expression}
% \end{figure*}

% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=0.99\linewidth]{fig/beat_close_up.pdf}
% \vspace{-0.5cm}
% \end{center}
%    \caption{\textbf{Qualitative Results on Facial expressions and Lip Sync by our Model Trained on the BEAT~\cite{{beat}} Dataset.} When provided with speech audio, our model produces facial expressions accompanied by precise lip shapes, as depicted in (a). Furthermore, (b) showcases diverse facial expressions, including eye blinking and eyebrow lifting.
%    }

% \label{fig:beat_face}
% \end{figure*}



% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=0.99\linewidth]{fig/beat_gesture.pdf}
% \end{center}
%    \caption{\textbf{Qualitative Results on the Gestures Synthesized by our Model Trained on the BEAT~\cite{{beat}} Dataset.} The characters skillfully utilize expressive and lifelike gestures to effectively communicate concepts like ``dream'', ``design'' and ``street''. They also employ rhythmic synchronization and emphasis, exemplified by gestures corresponding to ``never'' and ``some''.  
%    }

% \label{fig:beat_gesture}
% \end{figure*}



